BanditQ: Fair Bandits with Guaranteed Rewards

Classic no-regret multi-armed bandit algorithms, including the Upper Confidence Bound (UCB), Hedge, and EXP3, are inherently unfair by design. Their unfairness stems from their objective of playing the most rewarding arm as frequently as possible while ignoring the rest. In this paper, we consider a fair prediction problem in the stochastic setting with a guaranteed minimum rate of accrual of rewards for each arm. We study the problem in both full-information and bandit feedback settings. Combining queueing-theoretic techniques with adversarial bandits, we propose a new online policy, called BanditQ, that achieves the target reward rates while conceding a regret and target rate violation penalty of at most $O(T^{\frac{3}{4}}).$ The regret bound in the full-information setting can be further improved to $O(\sqrt{T})$ under either a monotonicity assumption or when considering time-averaged regret. The proposed policy is efficient and admits a black-box reduction from the fair prediction problem to the standard adversarial MAB problem. The analysis of the BanditQ policy involves a new self-bounding inequality, which might be of independent interest.

==> BwK.tex <==
\section{Bandit with Knapsack (\texttt{BwK})} \label{BwK}

We now consider the Bandits with Knapsacks (\texttt{BwK}) problem in adversarial environments in the full information set-up \citep{immorlica2022adversarial} in the Budget regime $B_T=\Omega(T)$. In particular, we consider a sequential model, where, starting from a sublinear amount of resource at the beginning, the $i$\textsuperscript{th} resource arrives at the deterministic rate of $0\leq \lambda_i \leq 1$ units per round. Clearly, our sequential model is strictly stronger than the static budget model where the entire budget $B_T$ is available before the game starts.

The action $\bm{x}(t)$ consumes $b_i(t)x_i(t)$ amount of resource $ i\in [N],$ and yields in an overall reward of $\langle \bm{r}(t), \bm{x}(t)\rangle = \sum_i r_i(t) x_i(t).$  Without any loss of generality, we assume that the reward $r_i(t)$ and the consumption $b_i(t)$ for each arm lie in the interval $[0,1], \forall t\geq 1.$   

\subsection{Characterization of the Optimal Offline Benchmark} \label{offline2} 
We compare the regret of the proposed \texttt{BanditQ} policy against reward accrued by any fixed distribution $\bm{x}^* \in \Delta_N$ over the experts while respecting the resource budget constraints. For this, \cite{badanidiyuru2018bandits} considers a linear relaxation where, at each round, the learner receives the same reward vector $\bm{r}(t)= \bar{\bm{r}}$ and the same consumption vector $\bm{b}(t)= \bar{\bm{b}}, \forall t\geq 1,$ where we define 
\begin{eqnarray} \label{benchmark_def}
	\bar{\bm{r}}\equiv\frac{1}{T}\sum_{t=1}^T \bm{r}(t), ~ \bar{\bm{b}} \equiv \frac{1}{T}\sum_{t=1}^T \bm{b}(t).
\end{eqnarray}  
Next, we find the optimal static distribution $\bm{x}^* \in \Delta_N$ for maximizing the cumulative reward as follows: 
\begin{eqnarray*}
	\texttt{OPT}_{\texttt{LP}}= \max_{\bm{x}} \sum_i \bar{r}_i x_i,
\end{eqnarray*}
Subject to
\begin{eqnarray} \label{opt_constr}
\bar{b}_i x_i \leq \lambda_i, ~\forall i \in [N].	
\end{eqnarray}
\citet[Lemma 3.1]{badanidiyuru2018bandits} showed that $\texttt{OPT}_{\textrm{FD}} \leq T\texttt{OPT}_{\textrm{LP}}.$ In this paper, we consider a weaker benchmark where the averaging in Eq.\ \eqref{benchmark_def} is done over all windows of size $w\geq 1,$ \emph{i.e.,}
 \begin{eqnarray} \label{benchmark_def2}
	 \bar{\bm{b}}_{w, \tau} \equiv \frac{1}{w}\sum_{t=\tau}^{\tau+w-1} \bm{b}(t).
\end{eqnarray}  
This leads us to consider the relaxed offline benchmark:
\begin{eqnarray*}
	\texttt{OPT}'_{\texttt{LP}}= \max_{\bm{x}} \sum_i \bar{r}_i x_i
\end{eqnarray*}
Subject to
\begin{eqnarray} \label{opt_constr2}
\bar{b}_{i,w, \tau} x_i \leq \lambda_i, ~\forall i \in [N], \forall \tau.	
\end{eqnarray}
Although the above benchmark could be weaker than $\texttt{OPT}_{\texttt{FD}}$,  on the flip side, the \texttt{BandiQ} policy is oblivious to the window size $w$ as long as it is constant (independent of $T$). 
\subsection{Policy design} \label{policy2}

 To each expert $i \in [N],$ we associate a non-negative state variable $Q_i(t),$ which evolves as follows:
\begin{eqnarray} \label{Q_ev2}
	Q_i(t)= \big(Q(t-1)+b_i(t)x_i(t)-\lambda_i\big)^+, ~Q_i(0)=0.
\end{eqnarray}
The intuition is that, any online policy $\pi^{\texttt{BwK}}=\{\bm{x}(t)\}_{t\geq 1}$, that stabilizes the queues, ensures that the rate of consumption of any resource is roughly bounded by the rate of generation or arrival. 
As before, we define the potential function 
\begin{eqnarray} \label{potential_def2}
	\Phi(\tau) = \sum_i Q_i^2(\tau), ~~\tau \geq 0.
\end{eqnarray}
From Eqn.\ \eqref{Q_ev2}, we have 
\begin{eqnarray*}
	Q_i^2(\tau) &\leq& \big(Q_i(\tau-1)+ b_i(\tau)x_i(\tau)-\lambda_i\big)^2 \\
	&\leq & Q_i^2(\tau-1) + x_i(\tau) + 1 + 2Q_i(\tau-1)\big(b_i(\tau)x_i(\tau)-\lambda_i\big),
\end{eqnarray*}
where, in the above inequality, we have used the fact that $b_i(\tau), x_i(\tau), \lambda_i \in [0,1].$ Summing up the above inequality over all experts $i \in [N],$ we obtain the following upper-bound on the change of potential 
\begin{eqnarray*}
	\Phi(\tau)-\Phi(\tau-1) \leq N+1 + 2\sum_{i \in [N]}Q_i(\tau-1)\big(b_i(\tau)x_i(\tau)-\lambda_i\big). 
\end{eqnarray*}
Fix any feasible fixed $\bm{x}^* \in \Delta_N$ which satisfies the resource conservation constraints $b_i(\tau) x_i^* \leq \lambda_i, \forall i \in [N].$ Let $\{V_\tau\}_{\tau\geq 1}$ be a non-negative non-deceasing sequence of real numbers. Define a surrogate prediction problem $\Xi$ where the reward for the $i$\textsuperscript{th} arm is defined as
\begin{eqnarray*}
	r_i'(\tau)= V_\tau r_i(\tau)- Q_i(\tau-1) b_i(\tau), ~~\forall i, \tau.
\end{eqnarray*}
Note that, unlike the original problem, the rewards in the surrogate problem $\Xi$ need not be bounded. 

\subsection{Analysis and Regret bounds}
Consider the following sequence of inequalities:
\begin{eqnarray} \label{main_eq2}
	&& \Phi(\tau)-\Phi(\tau-1) + 2V_\tau \big[\sum_{i} r_i(\tau)(x_i^* - x_i(\tau))\big] \nonumber \\
	&\leq& N+1 + 2\sum_i Q_i(\tau-1)(b_i(\tau)x_i^*-\lambda_i)+ 2\sum_i r_i'(\tau)(x_i^*-x_i(\tau)) \nonumber \\
	&\stackrel{(a)}{\leq} & N+1 + 2\sum_i r_i'(\tau)\big(x_i^*-x_i(\tau)\big),
\end{eqnarray}
where, in (a), we have used the feasibility of the offline benchmark $\bm{x}^*$ which has the property that $b_i(\tau)x_i^* \leq \lambda_i.$ Summing up \eqref{main_eq2} for $\tau=1$ to $\tau=t$ and recalling the definition of the quadratic potential function from \eqref{potential_def2}, we obtain:
\begin{eqnarray} \label{eq2}
	\sum_{i}Q_i^2(t) + 2\sum_{\tau=1}^tV_\tau\sum_i r_i(\tau)(x_i^*-x_i(\tau)) \leq (N+1)t + 2 \textrm{Regret}^{\Xi}_t.
\end{eqnarray}
Using the Online Gradient Ascent (OGA) policy for the surrogate problem, the regret term can again be bounded as:
\begin{eqnarray*}
	\textrm{Regret}_t^\Xi &\leq& 2 \sqrt{\sum_{\tau=1}^t ||\bm{r'}(\tau)||^2_2} \\
	&=& 2\sqrt{\sum_{\tau=1}^t \sum_i (V_\tau r_i(\tau)- Q_i(\tau-1) b_i(\tau))^2} \\
	&\stackrel{(a)}{\leq} & 2\sqrt{\sum_{\tau=1}^t \sum_i 2\big(V_\tau^2+ Q_i^2(\tau-1)\big) }\\
	&\stackrel{(b)}{\leq}& 2\sqrt{2 \sum_{\tau=1}^t \sum_i Q_i^2(\tau)} + 2\sqrt{2N\sum_{\tau=1}^t V_\tau^2}.
 \end{eqnarray*}
where in (a), we have used the fact that $(x-y)^2 \leq 2(x^2+y^2)$ and in (b), we have used the fact that $\sqrt{x+y} \leq \sqrt{x}+\sqrt{y}.$ Substituting the above regret bound in \eqref{eq2}, we obtain the following Eqn.\ 
\begin{eqnarray}\label{master_ineq}
	\sum_{i}Q_i^2(t) + 2\sum_{\tau=1}^tV_\tau\sum_i r_i(\tau)(x_i^*-x_i(\tau)) \leq (N+1)t +  4 \sqrt{2\sum_{\tau=1}^t\sum_{i} Q_i^2(\tau) } + 4\sqrt{2N\sum_{\tau=1}^t V_\tau^2},
\end{eqnarray}
which is identical to Eqn.\ \eqref{main_ineq} apart from the coefficient of $t$ in the first term of the RHS. Hence, using the same argument as before, we obtain the following results:

\begin{proposition}
	Set $V_t=V=\Theta(\sqrt{T}), 1\leq t \leq T.$ Then the \texttt{BanditQ} policy ensures the following
	\begin{eqnarray*}
		\textrm{Regret}_t = O(T^{3/4}), ~\textrm{and}~ \sum_{z=t-\tau+1}^t b_i(z) x_i(z) \leq \lambda_i \tau  + O(T^{3/4}), \forall 1\leq \tau \leq t \leq T.
	\end{eqnarray*}
\end{proposition}
The above shows that starting with a sublinear $O(T^{3/4})$ amount of budget at the beginning the \texttt{BanditQ} policy satisfies the resource consumption constraint for all time $1\leq t \leq T$ and achieves a sublinear regret of $O(T^{3/4})$ against all feasible offline static predictions. 


















==> algorithm_OLD.tex <==
\section{The Policy: \large{\texttt{BanditQ}}}  \label{algorithm}
In this section, we propose \texttt{BanditQ} - an online learning policy that solves the above constrained prediction problem. 
On a high level, we define a natural queueing dynamics to account for the rate constraints. Then we extend the drift-plus-penalty framework of \cite{neely2010stochastic} to simultaneously achieve a small regret and ensure that the long-term rate constraints are met for the users in the subset $\mathcal{P}.$ However, to make this approach work, we must adapt the stochastic full-information setting of \cite{neely2010stochastic} to the adversarial set-up with online information. This extension is non-trivial and requires a new proof and algorithmic technique, which is very different from the celebrated \texttt{Max-Weight} policy.

We associate a non-negative state variable $Q_i(t)$ corresponding to each user $i$ in the protected set $\mathcal{P}.$ Under the action of an online policy $\pi = \{\bm{x}(t)\}_{t \geq 1},$ the state variables in the set $i \in \mathcal{P}$ evolve according to the following queueing dynamics known as the Lindley recursion:
\begin{eqnarray} \label{q-ev}
	Q_i(t)=\big(Q_i(t-1)+ \lambda_i - r_i(t)x_i(t)\big)^+, ~Q_i(0)=0,
\end{eqnarray}
where we adopt the usual notation $(y)^+\equiv \max(0,y).$ To get an intuition on the above dynamics, imagine that on every round $t$ a fixed deterministic amount of work $\lambda_i$ arrives at the queue $Q_i.$ Then, under the action $\bm{x}(t)$ of an online policy, $\min(Q(t-1)+ \lambda_i, r_i(t) x_i(t))$ amount of work departs from $Q_i.$ Hence, any online policy stabilizing the queues satisfies the long-term rate requirements. However, since we are also interested in achieving a small regret, meeting the rate constraints alone is not enough (\emph{c.f.} \cite{huang2023queue}). Our online policy must also achieve a small regret in terms of cumulative rewards against feasible stationary policies given by \eqref{feas}. Towards this, we define the following quadratic potential function (\emph{a.k.a.} Lyapunov function in queueing theory):
\begin{eqnarray*}
	\Phi(t) = \sum_{i \in \mathcal{P}} Q_i^2(t).  
\end{eqnarray*}
We now upper-bound the change of potential under the action of a policy. We have 
\begin{eqnarray*}
	Q_i^2(t) &\leq& \big(Q_i(t-1)+ \lambda_i - r_i(t)x_i(t)\big)^2 \\
	&\leq& Q_i^2(t-1) + \lambda_i + x_i(t)+ 2Q_i(t-1)(\lambda_i - r_i(t) x_i(t)), 
\end{eqnarray*}
where we have used the fact that $0\leq \lambda_i, r_i(t), x_i(t) \leq 1, \forall i, t.$ Summing up the above inequality, we have the following expression for the change of potential on round $t$:
\begin{eqnarray} \label{potential_change}
	\Phi(t) - \Phi(t-1) \leq 2 + 2\sum_{i \in \mathcal{P}} Q_i(t-1)\big(\lambda_i - r_i(t) x_i(t)\big),
\end{eqnarray}
where we have used the fact that $\sum_i \lambda_i \leq 1, \sum_i x_i(t) \leq 1.$ Motivated by the drift-plus-penalty framework of \cite{neely2010stochastic}, we now define an instance of the online prediction problem $\Xi$ where the reward on round $t$ of the $i$\textsuperscript{th} user is defined as 
\begin{eqnarray} \label{reward_def}
	r'_i(t) \equiv \big(Q_i(t-1) + V_t\big)r_i(t), ~\forall i \in [N].
\end{eqnarray}
In the above $\{V_t\}_{t\geq 1}$ is a sequence of non-negative non-decreasing parameters to be fixed later. We set $\lambda_i=0, Q_i(t)=0, \forall t, \forall i \notin \mathcal{P}$. 
 %To recapitulate the information structure, the coefficients $Q_i(t-1)+V_t$ are known, but the reward vector $\bm{r}(t)$ is unknown to the online policy before it makes the decision $\bm{x}(t) \in \Delta_N$ on round $t$. 
 Intuitively, the surrogate reward $\bm{r}'(t)$ defined in \eqref{reward_def} strikes a balance between meeting the target rates (through the first term) and achieving a small regret (through the second term).
 Our proposed \texttt{BanditQ} policy simply uses any adaptive no-regret policy, \emph{e.g.,} Online Gradient Ascent (\texttt{OGA}) \cite{orabona2019modern} or \texttt{Squint} \citep{koolen2015second}, for the auxiliary problem $\Xi$ defined above. For simplicity, we use the \texttt{OGA} policy, which updates the sampling distribution as follows:
\begin{eqnarray} \label{oga-update}
	\bm{x}(t+1) \gets \Pi_{\Delta_N}\bigg(\bm{x}(t) + \frac{\bm{r}'(t)}{\sqrt{2 \sum_{\tau=1}^{t}||\bm{r}'(\tau)||_2^2}} \bigg),
\end{eqnarray}
where the reward sequence $\{\bm{r}'(t)\}_{t\geq 1}$ is defined in \eqref{reward_def}.
%, and the state variables $\{\bm{Q}(t)\}_{t \geq 1}$ evolve as in Eq. \eqref{q-ev}. 
In Eq.\ \eqref{oga-update}, $\Pi_{\Delta_N}(\cdot)$ denotes the Euclidean projection operator on the standard simplex $\Delta_N$. 
 In our analysis, we only need the following adaptive bound \cite[Theorem 4.14]{orabona2019modern} achieved by \texttt{OGA} on the regret for the problem $\Xi,$ which is defined by replacing the reward vector $\bm{r}(t)$ with $\bm{r}'(t)$ in Eq.\ \eqref{regret_def}:
\begin{eqnarray} \label{regret-bound}
	\textrm{Regret}^\Xi_t \leq 2 \sqrt{\sum_{\tau=1}^t \sum_i (Q_i(\tau-1)+V_\tau)^2r_i(t)^2} 
	\leq  2\sqrt{2\sum_{\tau=1}^t\sum_iQ_i^2(\tau) } + 2 \sqrt{2N\sum_{\tau=1}^t V_\tau^2},
\end{eqnarray}
   where we have used the fact that $0\leq r_{i}(t)\leq 1, \forall t,i$.

\subsection{Analysis and Regret Bounds}  
Since the state variables $\{\bm{Q}(t)\}_{t \geq 1}$ corresponding to the users in class $\mathcal{P}$ evolve according to the recursion \eqref{q-ev}, we do not immediately have explicit control of the magnitude of the reward vector $\bm{r}'(t)$ and the regret bound for the auxiliary problem $\Xi.$ To control the queue lengths, we take an indirect route by making use of the regret bound \eqref{regret-bound}. Consider any stationary action $\bm{x}^* \in \Omega$.
From Eq. \eqref{potential_change}, we have 
\begin{eqnarray*}
\Phi(\tau)-\Phi(\tau-1)  - 2V_\tau \sum_i r_i(\tau)x_i(\tau) 
\leq 2+ 2 \sum_i Q_i(\tau-1) \lambda_i -2 \sum_{i} \underbrace{(Q_i(\tau-1)+V_\tau) r_i(\tau)}_{r_i'(\tau)} x_i(\tau).
\end{eqnarray*}
%Changing the dummy variable from $t$ to $\tau$ and 
Summing up the above inequality from $\tau=1$ to $\tau=t$ and recalling that $\Phi(t)=\sum_i Q_i^2(t), \Phi(0)=0$, 
%from $\tau=1$ to $\tau=t$, 
we obtain: 
\begin{eqnarray} \label{main_ineq}
	&& \sum_{i} Q_i^2(t) + 2 \sum_{\tau=1}^t V_\tau \sum_i r_i(\tau) (x_i^*-x_i(\tau))  \nonumber \\
	&\leq& 2t + \underbrace{2 \sum_{\tau=1}^t \sum_{i} Q_i(\tau-1) \big(\lambda_i-r_i(\tau) x_i^* \big)}_{\leq 0 ~(\textrm{from Eq.}\ \eqref{feas})}+2\textrm{Regret}^{\Xi}_t \nonumber\\
	%&&+ \textrm{Regret}^{\Xi}_t \nonumber \\
	&\leq&  2t +  4 \sqrt{2\sum_{\tau=1}^t\sum_{i} Q_i^2(\tau) } + 4\sqrt{2N\sum_{\tau=1}^t V_\tau^2},
\end{eqnarray} 
where we have used the feasibility of $\bm{x}^*$ from Eq.\ \eqref{feas} and the adaptive regret bound from Eq.\ \eqref{regret-bound}. Next, we claim the following deterministic bound on the state variables $\{\bm{Q}(t)\}_{t \geq 1}$ by choosing a constant parameter sequence. 
%for a specific setting of the $\{V_t\}_{t \geq 1}$ sequence. 
\begin{proposition}\label{q_bd}
	Setting $V_t=V=\Theta(\sqrt{T}), \forall t\geq 1$, we obtain $Q_i(t) = O(T^{3/4}), \forall i \in \mathcal{P}, 1\leq t\leq T.$ 
\end{proposition} 
\begin{proof}
From Eq.\ \eqref{main_ineq}, we have that for all $i \in \mathcal{P}$ and all $t\geq 1:$
\begin{eqnarray} \label{ineq1}
	Q_i^2(t) \leq 2(V+1)t + 4 \sqrt{2\sum_{\tau=1}^t\sum_{i}Q_i^2(\tau) } + 4V \sqrt{2Nt},
\end{eqnarray}
where we have used the fact that $\sum_i r_i(\tau)(x_i(\tau)-x_i^*) \leq 1, \forall \tau.$ Furthermore, since $\lambda_i \leq 1,$ we trivially have $Q_i(\tau) \leq \tau, \forall i,\tau.$ We now improve upon this trivial upper bound by substituting it in Eq.\ \eqref{ineq1}, yielding:
\begin{eqnarray*}
	Q_i^2(t) \leq O(T^{3/2}) + O(T^{3/2})+ O(T) = O(T^{3/2}),  \forall i, t.
\end{eqnarray*}
\emph{i.e.,}
$Q_i(t)=O(T^{3/4}), \forall i, 1\leq t\leq T.$ 
%
%By substituting the above bound again in Eq.\ \eqref{ineq1}, we have the following improved estimate:
%\begin{eqnarray*}
%	Q^2_i(T) \leq 
%\end{eqnarray*}
\end{proof}
The following proposition shows that the rate constraints of the users belonging to the protected classes are met.
\begin{proposition} \label{rate-prop}
	Under the \texttt{BanditQ} policy with $V_t=V=\Theta(\sqrt{T}),$ for any interval $\mathcal{I} \subseteq [T]$ such that $T^{3/4}=o(|\mathcal{I}|),$ we have 
	\[\liminf_{|\mathcal{I}| \to \infty} |\mathcal{I}|^{-1}\sum_{t \in \mathcal{I}} r_i(t)x_i(t) 
	  \geq \lambda_i, ~\forall i \in \mathcal{P}.\]
\end{proposition}
\begin{proof}
	Upon expanding \eqref{q-ev}, we obtain the following well-known representation for the Lindley recursion: 
	\begin{eqnarray*}
		Q_i(t) = \max_{1\leq \tau \leq t}(0, \lambda_i \tau - \sum_{z=t-\tau+1}^t r_i(z) x_i(z)).
	\end{eqnarray*}
	Substituting the bound from Proposition \ref{q_bd} in the above, we have for any $1\leq t\leq T$ and any $1\leq \tau \leq t:$
	\begin{eqnarray*}
		\tau^{-1}\sum_{z=t-\tau+1}^t r_i(z) x_i(z) \geq \lambda_i  - O(\frac{T^{3/4}}{\tau}),
	\end{eqnarray*}
	which gives a finite-time rate guarantee for each user $i \in \mathcal{P}.$
	Hence, as long as $T^{3/4}/|\mathcal{I}| \to 0,$ we have
	\begin{eqnarray*}
		\liminf_{T \to \infty} |\mathcal{I}|^{-1}\sum_{t \in \mathcal{I}} r_i(t)x_i(t)  \geq \lambda_i, ~\forall i \in \mathcal{P}.
	\end{eqnarray*} 
\end{proof}
%Next we investigate the regret bound achieved by the \texttt{BanditQ} policy.
Using Proposition \ref{q_bd}, we now derive a sublinear regret bound achieved by the \texttt{BanditQ} policy. 
\begin{proposition} \label{regret_prop}
Upon setting $V_t=V=\Theta(\sqrt{T}), 1 \leq t\leq T,$ the \texttt{BanditQ} policy achieves $O(T^{3/4})$ regret as defined in Eq.\ \eqref{regret_def}:  
%	\begin{eqnarray*}
		%$\textrm{Regret}_T = O(T^{3/4}).$
%	\end{eqnarray*}
\end{proposition}
\begin{proof}
	Substituting the queue length bound from Proposition \eqref{q_bd} into the inequality \eqref{main_ineq} and using the fact that $Q_i^2(T) \geq 0, \forall i, t,$ we have 
	\begin{eqnarray*}
		%&&2V \textrm{Regret}_T \\
	2V \textrm{Regret}_T &\leq&  \sum_{i} Q_i^2(T) + 2V  \sum_{\tau=1}^T \sum_i r_i(\tau) (x_i^*-x_i(t)) \\ 
		&\leq& 2T + O(T^{5/4}) + O(T)= O(T^{5/4}). 
	\end{eqnarray*}
	Since $V=\Theta(\sqrt{T}),$ the above inequality immediately yields
	%\begin{eqnarray*}
		$\textrm{Regret}_T = O(T^{3/4}).$
	%\end{eqnarray*}
\end{proof}
%\vspace{-15pt}
 If one is only interested in satisfying the rate constraints while disregarding the cumulative rewards, the following proposition shows that the bound in Proposition \ref{q_bd} can be further improved to $O(\sqrt{t})$ by setting $V_t=0, \forall t.$ 
 \begin{proposition} \label{improved_bd}
 Setting $V_t=0, \forall t \geq 1,$ the state variables $\{\bm{Q}(t)\}_{t \geq 1}$ can be bounded as:
 \[Q_i(t) \leq 16\sqrt{kt}, ~\forall t\geq 1.\]
 \end{proposition}
 See Appendix \ref{improved_bd_proof} for the proof. 
%This implies a tighter finite-time bounds for the rate. 
%To show this, from Eq.\ \eqref{main_ineq}, we have:
%\begin{eqnarray} \label{new-eq}
%	Q_i^2(t) \leq 2t + 4 \sqrt{2\sum_{\tau=1}^t\sum_{i} Q_i^2(\tau) }~~ \forall t, \forall i \in \mathcal{P}.
%\end{eqnarray} 
%Substituting the trivial bound $Q_i(\tau) \leq \tau, \forall i, \tau,$ on the RHS of the above inequality, we have the following improved bound on the queue lengths:
%\begin{eqnarray*}
%	Q_i^2(t) \leq 2t+ O(t^{3/2}) = O(t^{3/2}),
%\end{eqnarray*}
%\emph{i.e.,} $Q_i(t) = O(t^{3/4}), \forall i,t.$ Plugging back the improved queue-length estimates in \eqref{new-eq}, we improve the bound further to $Q_i(t) = O(t^{5/8}), \forall i,t.$ Continuing this refinement process, we finally arrive at the bound $Q_i(t)= O(\sqrt{t}), \forall i \in \mathcal{P}, t.$ This result immediately improves the bound in Proposition \ref{rate-prop}, where we can take the averaging interval to be as small as $O(\sqrt{T}).$
%





















==> checklist.tex <==
\section*{Checklist}


 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [\textcolor{blue}{Yes}]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [\textcolor{blue}{Yes}]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [\textcolor{black}{No}]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [\textcolor{blue}{Yes}]
   \item Complete proofs of all theoretical results. [\textcolor{blue}{Yes}]
   \item Clear explanations of any assumptions. [\textcolor{blue}{Yes}]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Not Applicable]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Not Applicable]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Not Applicable]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Not Applicable]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Not Applicable]
   \item The license information of the assets, if applicable. [Not Applicable]
   \item New assets either in the supplemental material or as a URL, if applicable. [Not Applicable]
   \item Information about consent from data providers/curators. [Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}

==> introduction.tex <==
\section{Introduction}\label{intro}
%Consider the standard a
This problem has been considered in the learning literature with fairness constraints. 

==> related_work.tex <==
\section{Related Works} \label{related}
The papers \cite{alex, narahari-fair, wangbandit} considered the fair allocation problem in bandits in the stochastic setting. The paper \cite{huang2023queue} considered the scheduling problem in the adversarial setting for stabilizing queues. However, they do not consider the reward maximization problem under the queue stability constraints, which can be trivially solved in our setting by a randomized policy. 

==> statement_OLD.tex <==
\section{Introduction} \label{statement} 
In this paper, we consider the classic Prediction with Experts advice problem (\emph{a.k.a} the Prediction problem) in the adversarial setting with full information in the presence of rate constraints for pulling the arms. We present a new framework, based on elementary queueing theory to solve this problem. In particular, we consider two concrete problems, namely the Fair Experts problem and the Bandit with Knapsacks problem and show that how these problems can be simultaneously solved using the same queueing framework.  


Most of the learning algorithms deployed in practice aim to maximize the cumulative profit (\emph{e.g.,} the number of clicks on an ad). Consequently, they could end up discriminating against a subset of users the algorithm believes less rewarding. In a typical case of algorithmic discrimination, Facebook was sued for targeting ads on housing, credit and employment by race, gender, and religion - all protected classes under US law \cite{hao2019facebook}. A similar problem of fair allocation of resources arises in wireless scheduling, where schedulers maximizing the sum rate could result in not serving a subset of users having relatively poor channel conditions. The classic Proportional Fair scheduler solves the fair scheduling problem when the current channel conditions are known \cite{stolyar2005asymptotic}. However, maximizing the sum rate with user-specific rate constraints - a central problem in 5G network slicing remains open under unknown and adversarial channel conditions. In the context of online learning, several papers have considered the fair allocation problem in the stochastic setting. The paper \cite{huang2023queue} studied the scheduling problem in the adversarial environment in the context of stabilizing the queues. However, they do not consider the regret minimization problem under the queue stability constraints.
%, which can be trivially solved in our setting by a randomized policy. 

\subsection{Related work} \label{related_work}
The paper \cite{immorlica2022adversarial} uses a variant of the stochastic Bandit with Knapsack (\texttt{BwK}) policy to the adversarial setting. On the other hand, our policy is strictly tailored to the adversarial set up which, depends on the adaptive regret bound of the Online Gradient Descent policy. It is non-trivial and currently open whether a variant of our proposed policy can also be made to work in the stochastic set-up. 

\subsection{Technical Innovation} \label{techs}
To the best of our knowledge, all of the previously proposed online policies for the \BwK problem rely on the \emph{zero order} $O(\sqrt{T})$ regret bound of their online prediction subroutines. As an example, the algorithm proposed by \cite{immorlica2022adversarial} uses \texttt{EXP3.P} and \texttt{Hedge} as subroutines to their online primal-dual framework. On the other hand, our proposed \texttt{BanditQ} policy exploits a second-order regret bound that depends on the sum of squares of gradient components. A major obstacle with this approach is that the gradient components are not bounded a priori and depends on the past actions of the online policy itself. A key technical contribution of this paper is to simultaneously control both the norm of the gradients and the regret bound. We believe our proof technique is new and could be useful elsewhere.

%We consider the standard no-regret prediction problem with expert's advice in the adversarial setting with an additional long-term rate constraint for a subset of experts. 

%\textcolor{red}{Replace agents by users?}

 
%More specifically, we use the strong $(w, \epsilon)$-admissibility criterion with respect to a fixed schedule. The problem is interesting both in the full information and bandit setting and we tackle the full information version first. 

%We will also consider the simpler problem where there is a  given rate vector $\bm{r}$ such that arm $i$ must be pulled at least $r_i$ fraction of times. We seek a uniform algorithmic framework for both these problems. 


\section{Problem Formulation}  \label{model} 
In this paper, we consider the no-regret online prediction problem in the adversarial setting with an additional fairness constraint that requires that each agent in a protected class $\mathcal{P}$ must get a guaranteed rate of accrual of rewards, assuming the rates to be feasible. Formally, assume that there is a set of $N$ users, which on round $t$, receives the reward vector $\bm{r}(t),$ where $0\leq r_i(t) \leq 1, \forall i,t.$ On round $t$, an online prediction policy samples a user with a probability distribution $\bm{x}(t),$ where $\bm{x}(t)$ belongs to the standard probability simplex on $N$ atoms, denoted by $\Delta_N$. This short paper focuses on the full-information setting where the entire reward vector is revealed to the learner at the end of each round. Due to the action of the policy, the user $i$ receives an (expected) reward of $x_i(t)r_i(t), \forall i \in [N]$ and the online policy gets a reward of $\langle \bm{x}(t), \bm{r}(t) \rangle.$ Let $\mathcal{P} \subseteq [N]$ be a subset of $k$ users who belong to the \emph{protected classes}. We require that the long-term rate of rewards accrued by the $i$\textsuperscript{th} user in the class $\mathcal{P}$ must be at least $\lambda_i >0, \forall i\in \mathcal{P}.$ We emphasize that guaranteeing lower bounds to the rate of reward accruals of the individual users is different and more challenging than just constraining the frequency of sampling each user without considering their accrued rewards. To make the rate constraints feasible, 
%we assume that there is an offline probability distribution $\bm{x}^*$ over the users with the above property. 
we assume that there exists a feasible offline static allocation $\bm{x}^* \in \Delta_N$ that achieves the desired reward rates on all rounds. In other words, it is ensured that
\begin{eqnarray} \label{feas}
	x_i^* r_{i}(t) \geq \lambda_i, ~\forall i \in \mathcal{P}, ~\forall t \in [T].
\end{eqnarray}  
The above requirement can be compactly expressed as: 
\begin{eqnarray} \label{rate-requirement}
	x_i^* \geq \frac{\lambda_i}{\min_{1\leq t\leq T} r_i(t)},~ \forall i \in \mathcal{P}. 
\end{eqnarray}
Although the constraint in Eq.\ \eqref{rate-requirement} seems strong, considering a number of consecutive rounds at a time, our results hold even when the denominator in Eq.\ \eqref{rate-requirement} is replaced with the minimum rate averaged over any constant-sized window of size $w \geq 1.$ The proposed \texttt{BanditQ} policy is oblivious to the value of $w$.
The set of all feasible offline prediction distributions, given by the intersection of \eqref{rate-requirement} and the standard simplex $\Delta_N$, is denoted by $\Omega.$ The set $\Omega$ can be easily verified to be closed and convex having a diameter $D=\sqrt{2}.$ Our goal is to design an online user sampling policy $\{\bm{x}(t)\}_{t\geq 1}$ that achieves a sublinear regret against any benchmark in $\Omega$ over a horizon of a given length $T,$ \emph{i.e.,}
\begin{eqnarray} \label{regret_def}
	\textrm{Regret}_T \equiv \max_{\bm{x}^* \in \Omega}\sum_{t=1}^T \langle \bm{x}^*, \bm{r}(t)\rangle - \sum_{t=1}^T \langle \bm{x}(t), \bm{r}(t)\rangle,
\end{eqnarray}
while ensuring the long-term rate constraints. Formally, for any time interval $\mathcal{I} \subseteq [T]$, the rate constraint requires:
\begin{eqnarray*}
	\liminf_{|\mathcal{I}| \to \infty} |\mathcal{I}|^{-1}\sum_{t \in \mathcal{I}} r_i(t)x_i(t)  \geq \lambda_i, ~\forall i \in \mathcal{P}.  
\end{eqnarray*}
%In this paper, we will give a stronger \emph{uniform} guarantee of the reward rate achieved by our proposed policy.
We note two fundamental differences between the above problem and the standard Online Convex Optimization (OCO) framework \cite{orabona2019modern}. First, contrary to the OCO setting, where the benchmark set $\Omega$ is specified a priori independent of the rewards, in this problem, the set $\Omega$ depends on the rewards and remains unknown till the end of the horizon. Second, unlike the OCO setting, the action taken by the online policy on a round is not restricted to the set $\Omega$ provided that the long-term reward rate requirements of the protected classes are met.     
%Clearly, for the constraint \eqref{rate-requirement} to be feasible, it is 
The following conditions on rates are necessary and sufficient for ensuring feasibility \eqref{feas}: 
\begin{eqnarray} \label{nec-suff}
	\sum_{i \in \mathcal{P}} \frac{\lambda_i}{\min_{1\leq t\leq T} r_i(t)} \leq 1, ~\textrm{and} 
	~\lambda_i \leq \min_{1\leq t\leq T} r_i(t), \forall i\in \mathcal{P}.
\end{eqnarray}
In practice, the feasibility of a set of rate requirements can often be verified by assuming stationary rewards and using the historical reward data sequence. 
